RoAD Benchmark: How LiDAR Models Fail under Coupled Domain Shifts and Label Evolution

For 3D perception systems to operate reliably in real-world environments, they must remain robust to evolving sensor characteristics and changes in object taxonomies. However, existing adaptive learning paradigms struggle in LiDAR settings where domain shifts and label-space evolution occur simultaneously. We introduce \textbf{Robust Autonomous Driving under Dataset shifts (RoAD)}, a benchmark for evaluating model robustness in LiDAR-based object classification under intertwined domain shifts and label evolution, including subclass refinement, unseen-class insertion, and label expansion. RoAD evaluates three learning scenarios with increasing adaptation, from fixed representations (zero-shot transfer and linear probing) to sequential updates (continual learning). Experiments span large-scale autonomous driving datasets, including Waymo, nuScenes, and Argoverse2. Our analysis identifies central failure modes: (i) \textit{limited transferability} under subclass refinement and unseen-class insertion, and on non-vehicle class; and (ii) \textit{accelerated forgetting during continual adaptation}, driven by feature collapse and self-supervised learning objectives.

==> tab/cyclist_bicycle.tex <==
\begin{table}[h]
\caption{\textbf{Zero-shot transfer accuracy (\%) on nuScenes bicycle.}}
\centering
    \begin{tabular}{lr}
        \toprule
        \textbf{Total}                  & 70.2                  \\
        \midrule
        \textbf{bicycle.with\_rider}    & 100                  \\
        \textbf{bicycle.without\_rider} & 62.3                    \\ 
        \bottomrule
    \end{tabular}
    \label{tab:cyclist_bicycle}
    \vskip -0.1in
\end{table}
